On Lennard-Jones-type potentials on the half-line

In this paper we study a particle under the influence of a Lennard-Jones potential moving in a simple quantum wire modelled by the positive half-line. Despite its physical significance, this potential is only rarely studied in the literature and due to its singularity at the origin it cannot be considered as a standard perturbation of the one-dimensional Laplacian. It is therefore our aim to provide a thorough description of the Hamiltonian in one dimension via the construction of a suitable quadratic form. Our results include a discussion of spectral and scattering properties which finally allows us to generalise some results from [Robinson1974] as well as [RadinSimon1978].

==> 2sec.tex <==

\section{On the superconducting phase with surface pair interactions}
%
In the previous section we have seen that the superconducting phase in the bulk is destroyed through the presence of surface defects (see Theorem~\ref{TheoremDSNOn}). However, since the defects are imagined relatively small when compared to the bulk, (repulsive) interactions between the pairs should be taken into account for large pair surface densities. 

In order to account for those interactions, we pursue a (quasi) mean-field approach. More explicitly, the first term on the right-hand side of \eqref{HamiltonianFreeSecondQS} (i.e., the free Hamiltonian of the discrete graph) is replaced by
%
\begin{equation}\label{MeanFieldHamiltonian}
\sum_{j=1}^{n(L)}\lambda_{j}a^{\ast}_ja_j-\alpha N_{s}+\lambda \rho_{s}(\mu,L) N_{s}:=h_{MF}(\rho_{s},\alpha,\lambda)\ ,
\end{equation}
%
where $N_s:=\sum_{j=1}^{n(L)} a^{\ast}_ja_j$ is the associated number operator and 
%
\begin{equation}
\rho_{s}(\mu,L):=\frac{\omega^L_{\beta,\mu}(N_s)}{n(L)}
\end{equation}
%
the pair density on $\mathbb{C}^{n(L)}$. Furthermore, $\lambda > 0$ is the interaction strength associated with the repulsive interactions between the pairs in the surface defects.
%
\begin{remark}Note that the interaction term in the standard mean-field approach is $\lambda \frac{\hat{N}^2}{V}$ with $V$ the associated volume, see~\cite{MichVerbeure,VerbeureBook}.
	\end{remark}
%
Due to the nature of the interaction part in~\eqref{MeanFieldHamiltonian} we can rewrite it as
%
\begin{equation}
h_{MF}(\rho_{s},\alpha,\lambda)=\sum_{j=1}^{n(L)}\left(\lambda_{j}-\alpha+\lambda\rho_{s}(\mu,L) \right)a^{\ast}_ja_j
\end{equation}
%
which means that the corresponding eigenvalues $\{\lambda_j\}$ are effectively shifted by $\lambda\rho_{s}(L)-\alpha$. Accordingly, since the problem reduced to an effective non-interacting ``particle'' model, it means that the chemical potential is bounded from above by
%
\begin{equation}\label{RelationChemicalPotential}
\mu_{L} < \min\{\lambda\rho_{s}(\mu_L,L)-\alpha,E_0(L)\}\ ,
\end{equation}
%
taking into account that the lowest eigenvalue of the Laplacian is zero. Hence, $\mu_{max}(L)=\min\{\lambda\rho_{s}(\mu_L,L)-\alpha,E_0(L)\}$. Furthermore, the sequences of the chemical potentials $(\mu_{L})$ and the surface pair densities $(\rho_{s}(L))$ have to be chosen in a way such that
%
\begin{equation}\label{EquationI}
\rho=\lim_{L \rightarrow \infty}\frac{1}{L}\left(\sum_{j=1}^{n(L)}\frac{1}{e^{\beta\left[\left(\lambda_{j}-\alpha+\lambda \rho_{s}(\mu_L,L) \right)-\mu_{L}\right]}-1}+\sum_{n=0}^{\infty}\frac{1}{e^{\beta\left(E_n -\mu_{L}\right)}-1}\right)
\end{equation}
%
holds with
%
\begin{equation}\label{SurfaceDensityII}
\rho_{s}(\mu_{L},L)=\frac{1}{n(L)}\sum_{j=1}^{n(L)}\frac{1}{e^{\beta\left[\left(\lambda_{j}-\alpha+\lambda \rho_{s}(\mu_L,L) \right)-\mu_{L}\right]}-1}\ .
\end{equation}
%
%We rewrite~\eqref{EquationI} as
%
%\begin{equation}\label{EquationII}
%\rho_s(\mu_L,L)=\frac{L}{n(L)}\left(\rho-\frac{1}{L}\sum_{n=0}^{\infty}\frac{1}{e^{\beta\left(E_n %-\mu_{L}\right)}-1}\right)\ .
%\end{equation}
%
\begin{theorem}[Surface pair density] Let $(\mu_L) \in (-\infty,E_0(L))$ be a convergent sequence of chemical potentials with limit value $\mu < E_0$. Then 
	%
	\begin{equation}
	\lim_{L \rightarrow \infty}\left(\frac{n(L)}{L}\rho_s(\mu_L,L)\right)=\rho-\frac{1}{\pi}\sum_{n=1}^{\infty}\int_{0}^{\infty}\frac{1}{e^{\beta \frac{2\pi^2n^2}{d^2}}e^{\beta(x^2-\mu)}-1}\ud x\ .
	\end{equation}
	%
\end{theorem}
%
\begin{proof} Starting from~\eqref{EquationI}, the statement follows directly from formula~(3.4) in \cite{KernerElectronPairs} setting $\hbar=1$, $m_e=1/2$ and replacing $d$ by $d/\sqrt{2}$. Note here that this formula holds true also for a sequence of chemical potentials by uniform convergence.
\end{proof}
%
Now, if we assume that $\lim_{L\rightarrow \infty}\frac{L}{n(L)}=:\delta$ with $0\leq \delta \leq \infty$ then 
%
\begin{equation}\label{EquationLimitDensity}\begin{split}
\lim_{L \rightarrow \infty}\rho_s(\mu_L,L)&=\delta\left(\rho-\frac{1}{\pi}\sum_{n=1}^{\infty}\int_{0}^{\infty}\frac{1}{e^{\beta \frac{2\pi^2n^2}{d^2}}e^{\beta(x^2-\mu)}-1}\ud x\right)\\
&=:\rho_s(\mu,\delta)\ ,
\end{split}
\end{equation}
%
for $\mu_L \rightarrow \mu < E_0$. From a physical point of view it is now very interesting to write $\rho_s$ as
%
\begin{equation}
\rho_s(\mu,\delta)=\delta(\rho-\rho_{exc})\ ,
\end{equation}
%
where $\rho_{exc}=\rho_{exc}(\mu)$  equals the second term in brackets in~\eqref{EquationLimitDensity}. Note that $\rho_{exc}$ is the density of pairs occupying all excited states in the bulk in the thermodynamic limit.
%
\begin{lemma}[Destruction of the superconducting phase II]\label{ProofLemma}  If 
	%
	\begin{equation}
	\delta(\rho-\rho_{exc}) < \frac{E_0+\alpha}{\lambda}\ ,
	\end{equation}
	%
	then the superconducting phase in the bulk is destroyed.
\end{lemma}
%
\begin{proof} By relation~\eqref{RelationChemicalPotential} and the assumptions we conclude
	%
	\begin{equation}
	\mu <  E_0-\epsilon\ 
	\end{equation}
%
	for the limit point of $(\mu_L)$ for some constant $\epsilon > 0$. By Proposition~\ref{PropInfimumSpectrum} we get
	%
	\begin{equation}
	\lim_{L \rightarrow \infty}\frac{1}{L}\frac{1}{e^{\beta(E_0(L)-\mu_L)}-1}=0
	\end{equation}
	%
	which yields the statement .
\end{proof}
%
We immediately obtain the following statement which is interesting from a physical point of view.
%
\begin{cor}\label{CorollarySurface} Assume that $\delta=0$. Then, for all values $\lambda > 0$ of the interaction strength, the superconducting phase in the bulk is destroyed.
	
	More generally, if 
	%
	\begin{equation}
	\delta \cdot \rho < \frac{E_0+\alpha}{\lambda}
	\end{equation}
	%
 then the superconducting phase in the bulk is destroyed.
\end{cor}
%
\begin{remark} Corollary~\ref{CorollarySurface} means that the superconducting phase in the bulk is destroyed for arbitrarily large repulsive (quasi) mean-field interactions if the density of surface defects is large, i.e., of order larger than $L$.
	
	In addition, Lemma~\ref{ProofLemma} implies that the superconducting phase in the bulk is destroyed for arbitrarily large pair densities $\rho >0$ given the interaction strength $\lambda > 0$ is small enough or the ``surface tension'' $\alpha \geq 0$ large enough.
\end{remark}
%
Finally, we obtain the following result.
%
\begin{theorem}[Reconstruction of the superconducting phase] If $\delta > 0$ then there is a critical pair density $\rho_{crit}=\rho_{crit}(\beta,\alpha,\lambda) > 0$ such that for all pair densities $\rho > \rho_{crit}$ there exists a superconducting phase in the bulk.
\end{theorem}
%
\begin{proof} In a first step one chooses $\rho$, for given values $\beta,\alpha,\lambda > 0$, so large that
	%
	\begin{equation}\label{EQ1}
	\rho_s(E_0,\delta) > \frac{E_0+\alpha}{\lambda}\ .
	\end{equation}
	%
Then, using the same reasoning as in the proof of Lemma~\ref{ProofLemma} one now concludes that 
	%
	\begin{equation}\label{EQ2}
	\mu \leq E_0
	\end{equation}
	%
for the limit point of the sequence of chemical potentials, taking Proposition~\ref{PropInfimumSpectrum} into account.

Finally, using \eqref{EQ1} and \eqref{EQ2} in \eqref{SurfaceDensityII}, we conclude the existence of a constant $C > 0$ such that 
%
\begin{equation}
\sup_{\mu \in (-\infty,E_0]}|\rho_{s}(\mu,L)| < C
\end{equation}
%
for all $L\geq L_0$. This, however, contradicts~\eqref{EquationLimitDensity} when choosing a large enough pair density $\rho > 0$. As a consequence, the state $\varphi_0$ has to be macroscopically occupied in the thermodynamic limit and its contribution to~\eqref{EquationLimitDensity} has to be taken into account. 
\end{proof}
